Faster Algorithms for Fair Max-Min Diversification in $\mathbb{R}^d$

The task of extracting a diverse subset from a dataset, often referred to as maximum diversification, plays a pivotal role in various real-world applications that have far-reaching consequences. In this work, we delve into the realm of fairness-aware data subset selection, specifically focusing on the problem of selecting a diverse set of size $k$ from a large collection of $n$ data points (FairDiv). The FairDiv problem is well-studied in the data management and theory community. In this work, we develop the first constant approximation algorithm for FairDiv that runs in near-linear time using only linear space. In contrast, all previously known constant approximation algorithms run in super-linear time (with respect to $n$ or $k$) and use super-linear space. Our approach achieves this efficiency by employing a novel combination of the Multiplicative Weight Update method and advanced geometric data structures to implicitly and approximately solve a linear program. Furthermore, we improve the efficiency of our techniques by constructing a coreset. Using our coreset, we also propose the first efficient streaming algorithm for the FairDiv problem whose efficiency does not depend on the distribution of data points. Empirical evaluation on million-sized datasets demonstrates that our algorithm achieves the best diversity within a minute. All prior techniques are either highly inefficient or do not generate a good solution.

==> relatedwork.tex <==
\section{Related work}

==> response.tex <==
\section*{Response Letter for Paper 839}

We thank the reviewers for constructive reviews. We made all required changes and addressed the reviewers' comments.
Updates made in response to specific comments are color coded
(\ansa{Reviewer 1}, \ansb{Reviewer 2},
\ansc{Reviewer 3}, \ansmeta{Multiple reviewers and meta-reviewer}).
In summary, we made the following changes in this revision:
\begin{itemize}
    \item Instead of calling our algorithm MWU, we call it \newAlg{} (\textbf{M}ultiplicative weight update based \textbf{F}air \textbf{D}iversification).
    \item We improved the presentation by adding tables, figures, pseudocode, examples and by re-writing some parts of the technical algorithm.
    \item We implemented our algorithm for the streaming setting (SFairDiv problem) and ran experiments on real data. We also  added additional real-world examples to better motivate the SFairDiv problem.
    \item We added a table showing how many points are missed by our algorithm (Table~\ref{table:misspoints}).
    \item We added Figure~\ref{fig:skyline} showing that our method always returns a pareto-optimal solution.
    \item We explain FairGreedyFlow algorithm in more detail, and added a discussion comparing its running time with the running time of our method both in theory and in practice.
    \item Because of the space limit, we moved our algorithms that satisfy fairness with high probability to the technical report~\cite{techrep}. Hence, for simplicity, in the main part of the paper we focus on algorithms that satisfy fairness in expectation. We also moved the proofs of some lemmas in the technical report~\cite{techrep}.
\end{itemize}

\vspace{2em}
\mparagraph{Meta-reviewer}
\vspace{0.5em}
O1) Improve presentation according to R1O1, R2O2, R3O2, R3O4, R3O5, R3O6.

\ansmeta{Ans: We improved the presentation of our algorithms according to the reviews by R1, R2, and R3. Please check the changes in blue color in Section~\ref{sec:intro}, Section~\ref{sec:prelim}, and Section~\ref{sec:algs}.
We added tables, figures, examples, pseudocode, and re-wrote parts of the algorithms to improve the readability of the technical sections. The new structure for our main algorithm in Section~\ref{sec:algs} is the following: 
\begin{itemize}
    \item We first model our problem as a (new) linear feasibility problem ($\mathsf{LP}$\ref{lp:2}).
    \item Then, we show how we can write the new feasibility problem in the form of Equation~\eqref{feasibility}: $\exists x\in\mathcal{P}: Ax\leq b$ in order to be able to use the MWU method.
    \item We initialize an example explaining all central definitions that are needed for our algorithm.
\item Next, in paragraph ``New Algorithm'' we describe the overall algorithm (in a higher level) using the procedures $\mathsf{Oracle}(\cdot)$ and $\mathsf{Update}(\cdot)$ (for the MWU method), and $\mathsf{Round}(\cdot)$ to round the solution. After describing the algorithm, we show the overall running time as a function of the running times of all the procedures used in the algorithm.
\item Then, we design efficient near-linear time (more technical) algorithms for the procedures $\mathsf{Oracle}(\cdot)$, $\mathsf{Update}(\cdot)$, and $\mathsf{Round}(\cdot)$.
\item Each time we describe a new procedure we use our example to show the execution of the procedure in practice.
\end{itemize}
}
\vspace{0.5em}
O2) Better motivate the SFairDiv problem (R2O1).

\ansmeta{Ans: We added a few examples in Section~\ref{sec:intro} motivating the SFairDiv problem. SFairDiv is useful when data is generated in a streaming setting (for example, tweets or reviews) or when we have a large dataset that cannot fit in memory. Furthermore, in Subsection~\ref{subsec:streaming}, we implemented our algorithm for the SFairDiv problem and run experiments on real data comparing the efficiency (update time, post-processing time) and efficacy (diversity) of our method with other known streaming methods for the SFairDiv problem.}
\vspace{0.5em}

O3) Either better explain Figure 4 in text or use clearer visualization(s) to address R3O7.

\ansmeta{Ans: We have replaced the figure with Table~\ref{table:misspoints} showing the number of points missed by our algorithm with a clearer way.}
\vspace{0.5em}

O4) Shed light on the impracticality/inapplicability of k-center solutions to the problem at hand (R3O1).

\ansmeta{Ans: We added an example in Section~\ref{sec:related} showing why algorithms for the fair $k$-center problems cannot be used for the \fairDiv\ problem.}
\vspace{0.5em}

O5) Clarify the merits of MWU and why it would be the approach of preference compared to alternatives (R2O3)

\ansmeta{Ans: We added a discussion about it in Section~\ref{sec:experiments} and further highlight the key takeaways showing why our algorithm is better compared to the alternative methods. Furthermore, we run more experiments and added Figure~\ref{fig:skyline} showing that our method always returns a pareto-optimal solution and provides the best balance between running time and diversity.}
\vspace{0.5em}

O6) Better explain the FairGreedyFlow algorithm and how it compares with the current proposal (R1O2 lists specific questions on this that need be clarified)

\ansmeta{Ans: We added Table~\ref{table:results} showing the comparison of our new algorithm with state--of--the--art (including FairGreedyFlow). We also added a discussion about FairGreedyFlow in Section~\ref{sec:prelim} and Section~\ref{sec:experiments}.}

\vspace{0.5em}
O7) Add an explanation in the paper (akin to the one given in feedback) about the observed vs. theoretical complexity misalignment spotted in R2O4. Also, address R3O3 regarding the log n factors.

\ansmeta{Ans: In Section~\ref{sec:experiments}, we added a paragraph called ``Comparison of \newAlg{} and FairGreedyFlow'' comparing (and explaining) the running time of \newAlg{} and FairGreedyFlow, both in theory and in practice. Finally, we added the $\log n$ factors in Subsection~\ref{subsec:contr} (Contributions).}
\vspace{2em}

\mparagraph{Reviewer 1}
\vspace{0.5em}
O1) [OVERALL PRESENTATION] The paper comes with numerous theoretical and technical contributions. Although they are explained and discussed in detail, somehow they are still presented in a bit confusing way, or, at least, in a way that may make a reader get lost easily. Basically, the paper is plenty of verbose text to present them, and it is poor of concise summaries and synthetic but effective presentations. here are a few suggestions to help readability in this regard (these are only some possible options, if the authors come with better solutions/actions, that would still be good):
- Add a table where, for every setting (i.e., diversity in expectation, diversity with high probability, and so on, along with the various extensions), it is reported the state-of-the-art result (i.e., algorithm achieving approximation factor X, running in Y time and Z space) and the result achieved in the paper.
- Add a pseudocode summarizing the main proposed algorithm (i.e., the one ultimately used in the experiments), perhaps including the implementation variations discussed in Section 6.
- Add a clear and concise list (via bullet points, or in a table) that summarizes all the theoretical results of the paper (i.e., Algorithm X for Problem Y, achieving approximation Z, and taking time T and space S).

\ansa{Ans: We made all the suggested changes. In particular, we added Table~\ref{table:results} comparing our algorithms with the state-of-the-art. We added pseudocode for our main algorithm and all the sub-procedures we use. We also added a more concise list of our results in Subsection~\ref{subsec:contr}(Contributions). Furthermore, we added figures and examples to show the  execution of all our algorithms in detail. Finally, we made several minor changes in the descriptions of the algorithms that make them easier to follow. Please see Meta-reviewer O1.}

\vspace{0.5em}
O2) [RELATED WORK] The relationship to the Fair-Greedy-Flow algorithm in [7] is only barely discussed in Section 7. But Fair-Greedy-Flow deserves a more detailed discussion, as it runs faster than or comparably to the proposed algorithm. How does the design principles of the proposed algorithm conceptually compare to the ones of Fair-Greedy-Flow? How do the theoretical approximation, running time, and space of the proposed algorithm compare to the ones of Fair-Greedy-Flow?

\ansa{Ans: We added Table~\ref{table:results} showing the comparison of FairGreedyFlow with our new algorithm. We also added a discussion about FairGreedyFlow in Section~\ref{sec:prelim}. Finally, in Section~\ref{sec:experiments} we added a paragraph called ``Comparison of \newAlg{} and FairGreedyFlow'' comparing the running time of \newAlg{} and FairGreedyFlow, both in theory and in practice.}
\vspace{0.5em}


M1) Abstract: n, k are not defined.

M2) Section 3.1: "we we use"

M3) Section 6: "heath statistics" -> "health statistics"

\ansa{Ans: We made all the suggested minor changes.}

\vspace{3em}

\mparagraph{Reviewer 2}
\vspace{0.5em}

O1. One concern I have regards the motivation behind the SFairDiv problem. This problem makes sense in theory, but I believe the paper can benefit from an explanation of its practical applications in relation to database systems. The usefulness of FairDiv and QFairDiv is convincingly argued, but the use-cases for these problems do not necessarily translate to SFairDiv.

\ansb{Ans: We added a paragraph in Section~\ref{sec:intro}, showing new practical applications of the SFairDiv problem. SFairDiv is useful when data is generated in a streaming setting (for example, tweets or reviews) or when we have a large dataset that we cannot even store in memory. Furthermore, we implemented our streaming algorithm for the SFairDiv problem and run new experiments on real data in Subsection~\ref{subsec:streaming}. Please also check our response for Meta-reviewer O2.}

\vspace{0.5em}
O2. The paper presumes readers possess a solid theoretical computer science background, a presumption that may limit its accessibility. The general SIGMOD audience, which includes a diverse range of expertise, might find the content challenging to fully comprehend.

\ansb{Ans: We re-wrote parts of the paper, and added tables, figures, examples and pseudocode to improve the readability. Please check our response for R1O1 and Meta-reviewer O1.}

\vspace{0.5em}

O3. This is probably the most serious concern. The proposed method does not appear to be an obvious winner in the experiments. In fact, the experimental comparison lacks a clear "yardstick". If diversity is the number one concern (which I believe it should), than both FMMD-S and SFDM-2 are both more superior to MWU. If running time is the number one concern (which I do not believe it should), then MWU loses to many methods. This creates confusion as to what are the real practical merits of MWU.

\ansb{Ans: We added a discussion about it in Subsection~\ref{subsec:endendres}, last two paragraphs before the ``Proportional size'' paragraph.
Generally, a good algorithm for the FairDiv problem is a fast enough algorithm that returns a diverse enough set of points. Indeed, FMMD-S and SFDM-2 return more diverse results however they are very slow (20X or even 60X slower) and they do not even finish for some datasets. On the other hand, FairFlow and FairGreedyFlow are faster, but the sets they return have a much worse diversity (our algorithm returns $2$ or even $3$ times more diverse sets in all datasets).
Overall, our algorithm achieves the best tradeoff between diversity and time. Every other algorithm is either too slow (no result within 100 sec) or the diversity is too low (5 times worse than the best one). In order to emphasize that our algorithm (\newAlg{}) provides the best balance between diversity and running time, we added Figure~\ref{fig:skyline}. We fix $k=100$, and for every algorithm we plot the running time and the diversity of the returned set as a point in the plane. An algorithm returns a \emph{pareto-optimal} result if there is no other algorithm that returns a more diverse set faster. Our algorithm always returns a pareto-optimal result. In fact, only our algorithm (\newAlg{}) and FairFlow always return a pareto-optimal result. Fairflow returns a pareto-optimal result because it is the fastest algorithm, however it returns sets with arbitrarily bad diversity in some cases (for example check Figure~\ref{fig:diverse:equal} (b) and (c)). Hence, we conclude that our algorithm always provides the best balance between diversity and running time compared to all other baselines.

%A good algorithm should be competitive in both quantities. MWU returns a pareto-optimal solution, i.e. no other algorithm returns a more diverse set, faster. FMMD-S and SFDM-2 indeed return more diverse results, however for some datasets they do not even finish, or they take 20X more time than our algorithm. At the same time, FairFlow and FairGreedyFlow indeed are faster, but the sets they return have a much worse diversity. Although our algorithm is slightly slower than the fastest algorithms for FairDiv – it scales to large datasets, and returns sets with high diversity in reasonable time. Overall, it achieves the best tradeoff between diversity and time. Every other algorithm is either too slow (no result within 100 sec) or the diversity is too low (5 times worse than the best one).
}

\vspace{0.5em}

O4. The authors' MWU algorithm runs in $O(nlog(k) + mk^2log^3(k))$ time. This is better than the FairGreedyFlow algorithm [7], which takes $O(kn + (mk)^2.37)$ time. However, in Figures 6 and 8, FairGreedyFlow is almost (except for the Census dataset in Figure 8) consistently faster than MWU. The authors did not explain why the experimental evaluation fails to support theory

\ansb{Ans: In Section~\ref{sec:experiments} we added a paragraph called ``Comparison of \newAlg{} and FairGreedyFlow'' comparing and explaining the running time of \newAlg{} and FairGreedyFlow, both in theory and in practice. Please also check R1O2.}

\vspace{0.5em}

Minor:
In Thm 2.2, should the second occurrence of "ORACLE" be "$\rho$-ORACLE"?

\ansb{Ans: Indeed, thank you for the careful reading. We changed it.}

\vspace{3em}

\mparagraph{Reviewer 3}

\vspace{0.5em}

O1) Related Work: A statement has been made that there is a strong connection to k-center clustering and that some (greedy) algorithms achieve the same approximation, but that it is unclear if algorithms for the k-center clustering problem can be applied to solve fair max-min diversification. It is briefly mentioned, that the optimal solution of one problem can be arbitrarily bad for the other, but it is not made clear. A small example might help to clarify that. Minor: Additional information on why FairMaxSum algorithms cannot be transferred to FairDiv would be helpful (or a reference to a paper that shows that issue).

\ansc{Ans: In Section~\ref{sec:related}, we added an example in $\Re^1$ showing that an optimum solution for the fair $k$-center problem can be arbitrarily bad for the \fairDiv\ problem. For the comparison between FairMaxSum and \fairDiv\ we added some citations that have already highlighted the differences.}

\vspace{0.5em}

O2) Some details in Sec. 1.1 should be moved to other sections as some information is too much for this section. The introduction should focus on the motivation and contributions. For instance, Coresets are introduced with some details, and related work is introduced that is not needed in this section.

\ansc{Ans: We re-wrote a more concise version of Subsection~\ref{subsec:contr}.  We removed all citations and we moved the definition of the coreset before Subsection~\ref{subsec:contr}. We had to move the coreset definition before Subsection~\ref{subsec:contr}, because in Subsection~\ref{subsec:contr} we state our new result, that any approximation algorithm for the $k'$-center clustering problem can be used to derive a coreset for the \fairDiv\ problem. This is a new and interesting result on its own. Then the coreset is used to accelerate our algorithm.
%Our goal was to give the main results along with the main ideas to derive them. If the current version of Subsection~\ref{subsec:contr} is still technical we are happy to only keep our results and completely remove the main ideas from this section.
}

\vspace{0.5em}

O3) In Contributions, the authors mention that log n factors are ignored, but if they affect the time complexity, then this is important.

\ansc{Ans: We added all $\log n$ factors in Contributions. In the new Table~\ref{table:results}, we skipped the $\log n$ factors because they do not affect the comparison and it simplifies the table. If needed, we can definitely add the $\log n$ factors in the table as well.}

\vspace{0.5em}

O4, O5) Use cases/examples/figures would be helpful in fully understanding the approach. As it is written, it is quite hard to follow, especially for readers without detailed background knowledge to fully appreciate the "proofs" of the paper.
Some of the claims are hard to grasp, which might be due to to the over-technical and dense presentation (relates to O4). Some more explanation/rationale for central definitions would be useful.

\ansc{Ans: We re-wrote parts of the paper, we added tables, figures, pseudocode and examples to improve the readability. Please also check our response for Meta-reviewer O1 and R1O1.}

\vspace{0.5em}

O6) Key Takeaway (2) should be rephrased. Although SFDM-2 and FMMD-S take longer than MWU (according to experiments), "40x" is not always accurate, only in some cases (e.g., for $k=20$ on the Diabetes dataset it seems to be around 20x and 30x while on the Census dataset, it is roughly 60x and 100x respectively for SFDM-2 and FMMD-S). The key takeaways should hold in general.

\ansc{Ans: We thank the reviewer for the observation. We replaced Key Takeaway (2) with a more precise argument.}

\vspace{0.5em}

O7) As the returned color distribution might not fulfill all constraints completely, it would be interesting to show how many points are missed compared to state-of-the-art approaches (e.g., by comparing the bottleneck color values for each approach).

\ansc{Ans: We replaced the Figure we had, with Table~\ref{table:misspoints} and added a discussion about it in the end of Subsection~\ref{subsec:micro}. In Table~\ref{table:misspoints}, we show the number of missing points per color (on average after $5$ executions of our algorithm) in Diabetes (left) and Popsim (right) datasets for \newAlg{}-$0.1$ and \newAlg{}-$0.3$. 
For $\stopping=0.3$, our algorithm rarely misses a point. For the Diabetes dataset it never misses a point. For the Popsim dataset, the maximum average number of points it misses for a group is $1.4$ (this is also the case in all other datasets we tried). For each $k$ it misses on average $1.16$ points in total, over all groups. 
The other baselines in the experiments do not miss any point, so we did not add them in this table.


%This is what we were trying to show in Figure 4. For two representative datasets, for every k, we show two bars: the left one shows the real number of points from each color (as a fraction), while the right one shows the fraction of points for each color returned by MWU. For g=0.3 our algorithm rarely misses a point. It only happens sometimes when k is large. If Figure 4 is not clear, we can add more details, or add a different figure showing the absolute number of points missed for every k.
}

\vspace{0.5em}

O8) While the extensions of FairDiv are discussed, they are left out of the experiments section. If these are important contributions, they should be properly evaluated as well. Given points raised before, I would suggest to possibly remove these extensions from the paper to free up some space to more properly discuss the main technical contribution of the paper.

\ansc{Ans: We implemented our algorithm for the SFairDiv problem and run experiments on real data in Subsection~\ref{subsec:streaming}. Furthermore, we show new practical applications of the SFairDiv problem in Section~\ref{sec:intro}. Please also check R2O1.}

\vspace{0.5em}

M1) In "1.1 Contributions", Section 5 should be referred to in paragraph 4.

\ansc{Ans: We added it.}

M2) The gap between subcaption and caption of Figure 1 is too small.

\ansc{Ans: We increased the gap.}

M3)The y-axis requires more information in the depicted figures. While I expect the runtime to be measured in $s$, it is not defined what the measurement uses.

\ansc{Ans: We added (sec) on the $y$-axis of runtime.}

M4) At the end of Section 6.1, the authors mention that in the following experiments $g = 0.3$ (due to showing the high-quality results for a reasonable runtime). Thus, for the other experiments, the approach is only named ``MWU''. For consistency, I would keep the same label ``MWU 0.3'' within the figure legend and only discard the value for the discussion.

\ansc{Ans: We made this change. Please notice that we changed the name of our algorithm to \newAlg{} so we use \newAlg{} ($g=.3$) in the figure legend.}

M5) Consider renaming your method to be more precise as it simplifies referring to your approach in upcoming research. MWU is one core method used within your approach, so naming your algorithm ``MWU'' might be misleading.

\ansc{Ans: We changed the name of new algorithm to \newAlg{}. We also call the streaming version of our algorithm \newStreamAlg{}.}
